Defending Against Adversarial Denial-of-Service Data Poisoning Attacks

Data poisoning is one of the most relevant security threats against machine learning and data-driven technologies. Since many applications rely on untrusted training data, an attacker can easily craft malicious samples and inject them into the training dataset to degrade the performance of machine learning models. As recent work has shown, such Denial-of-Service (DoS) data poisoning attacks are highly effective. To mitigate this threat, we propose a new approach of detecting DoS poisoned instances. In comparison to related work, we deviate from clustering and anomaly detection based approaches, which often suffer from the curse of dimensionality and arbitrary anomaly threshold selection. Rather, our defence is based on extracting information from the training data in such a generalized manner that we can identify poisoned samples based on the information present in the unpoisoned portion of the data. We evaluate our defence against two DoS poisoning attacks and seven datasets, and find that it reliably identifies poisoned instances. In comparison to related work, our defence improves false positive / false negative rates by at least 50%, often more.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations
	       

==> old_main/old_main.tex <==
% \documentclass{article}


% \usepackage{arxiv}

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{graphicx}
% \usepackage{subcaption}

% \title{Defending Against Adversarial Denial-of-Service Data Poisoning Attacks}

% \author{
% Simon Roschmann\thanks{Authors contributed equally}\\
% Cognitive Security Technologies\\
% Fraunhofer AISEC\\
% 85748 Garching, Germany\\
% \texttt{simon.roschmann@tum.de}\\
% \And
% Nicolas M. Müller\footnotemark[1]\\
% Cognitive Security Technologies\\
% Fraunhofer AISEC\\
% 85748 Garching, Germany\\
% \texttt{nicolas.mueller@aisec.fraunhofer.de}\\
% \And
% Konstantin Böttinger\\
% Cognitive Security Technologies\\
% Fraunhofer AISEC\\
% 85748 Garching, Germany\\
% \texttt{konstantin.boettinger@aisec.fraunhofer.de}\\
% }

% \begin{document}
% \maketitle

% \begin{abstract}
% Data poisoning is one of the most relevant security threats against machine learning and data-driven technologies. 
% Since many applications rely on untrusted training data, an attacker can easily craft malicious samples and inject them into the training dataset in order to degrade the performance of machine learning models. 
% As recent work has shown, such Denial-of-Service (DoS) data poisoning attacks are highly effective.

% To mitigate this threat, we propose a new approach of detecting DoS poisoned instances.
% % defence mechanism which can reliably identify poisoned samples within a given classification dataset and allows the defender to remove malicious data.
% In comparison to related work, we deviate from clustering and anomaly detection based approaches, which often suffer from the curse of dimensionality and arbitrary anomaly threshold selection.
% Rather, our defence is based on extracting information from the training data in such a generalized manner that we can identify poisoned samples based on the information present in the unpoisoned portion of the data.
% We evaluate our defence against two DoS poisoning attacks and six datasets, and find that it identifies poisoned instances with high accuracy (FPR = 0.023, FNR = 0.022).
% \end{abstract}


% % keywords can be removed
% \keywords{Adversarial Machine Learning \and Denial-of-Service Data Poisoning \and Defence against Data Poisoning}

% \section{Introduction}\label{s:introduction}
% In recent years, machine learning has led to new opportunities and tremendous breakthroughs in the fields of image classification \cite{he2016deep, zoph2018learning} and speech recognition \cite{graves2013speech, xiong2016achieving}.
% Machine learning has also been applied in security-sensitive applications including face  recognition \cite{sun2014deep}, fingerprint identification \cite{wang2014fingerprint}, autonomous driving \cite{huval2015empirical} and the detection of spam, malware and network intrusion \cite{nelson2008exploiting, saxe2015deep, javaid2016deep}.

% However, machine learning models are vulnerable and can be targeted by attackers. \cite{huang2011adversarial} has created a taxonomy for adversarial machine learning that distinguishes between causative (poisoning) attacks compromising the learning mechanism at train time and exploratory (evasion) attacks circumventing the learning mechanism at test time.
% Evasion attacks exploit blind spots in the classifier that allow malicious activities to remain undetected, e.g. test samples are manipulated to be misclassified at run time. 
% \cite{biggio2013evasion} show how changing malicious \emph{pdf} files can make them look legitimate and prevent detection by the classifier.

% In contrast, poisoning attacks manipulate train data to compromise the integrity or availability of a classifier. 
% These can be separated into back-door and Denial-of-Service (DoS) attacks.
% When performing back-door poisoning, the attacker creates a backdoor during training that allows control over the model at test time.
% \cite{chen2017targeted} evaluate back-door poisoning against facial recognition systems and demonstrate for example how an adversary can bypass authentication by forging his identity as the target person in a system. 
% DoS poisoning attacks also occur during training and aim at maximally degrading the performance of a model to make an application or service unusable. 
% \cite{nelson2008exploiting} show that sending attack emails, which contain many words likely to occur in legitimate emails, can increase the likeliness of future benign emails to be marked as spam by the learning algorithm.
% Causing an incorrect distinction between malicious and legitimate emails makes a spam filter unusable.
% Further poisoning attacks are explored in \cite{munoz2017towards, biggio2011support, biggio2012poisoning, xiao2015feature, koh2017understanding} and considered to be one of the most significant threats for systems that rely upon collecting untrusted data.

% To mitigate the threat of DoS poisoning, previous work has developed defences based on measuring the influence of samples on a model \cite{nelson2008exploiting, koh2017understanding} or on clustering and anomaly detection \cite{paudice2018detection, paudice2018label}. 
% Most defences are computationally inefficient or suffer from the curse of dimensionality \cite{Keogh2017}, which states that the sparsity of data in high dimensional space makes the search for similarity complicated. 
% Also, anomaly detection based approaches often suffer from arbitrary selection of detection thresholds.

% \textbf{Contribution.}
% The main contribution of this paper is a new defence against strong DoS poisoning attacks, such as poisoning attacks with back-gradient optimization presented in \cite{munoz2017towards}.
% Our defence is based on the re-evaluation of training samples by the poisoned classifier, which leverages the information present in the unpoisoned part of the dataset to identify and iteratively remove the poison instances.
% No interaction with a human oracle is required.
% This approach overcomes difficulties and constraints of previously proposed defences. 
% Compared to outlier detection, our approach is not susceptible to the curse of high dimensionality. 
% Moreover, we do not put any constraints on the datasets, do not require knowledge about the fraction of poison samples within our training dataset and do not restrict our defence to linear or binary models.
% An experimental evaluation of two poisoning attacks against the classification of six datasets with neural networks shows the effectiveness of our proposed defence methodology.

% The paper is organized as follows: In Section \ref{s:related_work}, we discuss related work. 
% Section \ref{s:poisoning_attack} summarizes the threat model and presents state-of-the-art attacks against which we evaluate our proposed defence.
% Section \ref{s:poisoning_defence} introduces our defence, while Section \ref{s:empircal_eval} presents experimental results which demonstrate the effectiveness of the evaluated attacks and our defence. 
% Finally, we conclude the paper in Section 6 and discuss further work.

% \section{Related Work}\label{s:related_work}
% Poisoning attacks and defences have been explored against general machine learning algorithms and practical applications. 
% Previous attacks have mainly considered binary classification tasks, while previous defences have primarily applied outlier detection.

% \subsection{Poisoning Attack}\label{ss:poisoning_attack}
% A practical DoS poisoning attack against spam filters is presented in \cite{nelson2008exploiting}. Sending attack e-mails that contain many words likely to occur in legitimate messages can compromise a machine learning spam filter and prevent the victim from seeing future legitimate e-mails.

% Simple label flipping poisoning attacks against the binary classification with Support Vector Machines are proposed in \cite{biggio2011support}.
% To maximize the classification error, the attacker chooses a subset of influential poison samples by evaluating the impact of samples with flipped labels on a separate validation set.
%  \cite{biggio2012poisoning} have been the first to demonstrate a poisoning attack strategy against Support Vector Machines by solving a bi-level optimization problem (see Equation~\ref{eq:1},~\ref{eq:2}) using the Karush-Kuhn-Tucker (KKT) conditions. 
%  \cite{xiao2015feature} apply the same approach to successfully poison Ridge regression, Lasso regression and Elastic Net regression.
% The use of influence functions is discovered in \cite{koh2017understanding} to measure the impact that a training sample has on the classifier's loss without performing computationally expensive retraining. 
% In the context of data poisoning this approach can be used to identify samples that should be modified to maximally compromise the classifier's performance.

% While all these approaches have focused on binary classification, \cite{munoz2017towards} target gradient-based deep learning algorithms for multiclass classification. 
% They extend the commonly used threat model to multiclass classification by introducing the concept of error specificity and overcome limitations regarding computation, memory and accuracy of poisoning attacks based on KKT conditions. 
% An empirical evaluation of the proposed poisoning algorithm with back-gradient optimization shows the significant degradation of classifiers when only a small fraction of training instances is controlled.

% \subsection{Poisoning Defence}\label{ss:poisoning_defence}
% To mitigate the threat of DoS poisoning attacks against spam filters, \cite{nelson2008exploiting} propose to measure the impact of each training sample on the classifier's performance. This defence can effectively determine samples that decrease the accuracy and should be discarded. 
% However, it is computationally expensive due to the many required steps of retraining and can suffer from overfitting when the dataset is small compared to the number of features.
% A similar, but more efficient approach is based on influence functions investigated in \cite{koh2017understanding}. 
% In the context of data poisoning, influence functions can be used to efficiently identify malicious instances that negatively impact the performance of a model.

% \cite{feng2014robust} propose a two step defence strategy for logistic regression classification. 
% After applying outlier detection, the algorithm is trained solving an optimization problem based on the sorted correlation between the classifier and the labels. 
% This approach is not feasible in practice as the fraction of poison samples is required for the algorithm to perform well.

% An effective and computationally efficient countermeasure for poisoning attacks against linear classifiers is demonstrated in \cite{paudice2018detection} based on data pre-filtering with outlier detection. 
% Although outlier detection in high-dimensional space is challenging, especially when the number of samples is small compared to the number of features, they demonstrate that even distance based outlier detection techniques mitigate the effect of optimal poisoning attacks.
% A defence against aggressive label flipping poisoning attacks is investigated in \cite{paudice2018label}.
% After flipping labels to maximize the loss function, a kNN-based outlier detection is applied to identify poisoned samples far from their genuine samples with the same label and relabel them correctly.

% Our defence improves upon related work as follows:
% \begin{itemize}
%     \itemsep0em
%     \item It is computationally light, as opposed to the defence in \cite{nelson2008exploiting}, which requires model retraining for every single sample.
%     Given a dataset with $n=1000$ instances, their algorithm requires fitting a model $1000$ times, while our defence only needs fitting a model twice.
%     \item Our defence is not susceptible to the curse of dimensionality, such as~\cite{paudice2018detection, paudice2018label}.
%     \item It does not require the correct percentage of poison samples $p$ (as opposed to e.g.~\cite{feng2014robust}), but in fact provides an estimate $\hat{p}$.
% \end{itemize}

% \section{Poisoning Attack}\label{s:poisoning_attack}
% In this section we present the DoS poisoning attacks against which we evaluate our defence.
% We choose a label flipping attack as baseline, and an attack based on back-gradient optimization as presented in \cite{munoz2017towards}.
% We feel that the chosen attacks are representative for the general class of Denial-of-Service data poisoning attacks, of which there are indeed only a few (see Section \ref{s:related_work}).

% \subsection{Threat Model}\label{ss:threat_model}
% The taxonomy for attacking machine learning algorithms has originally been  presented in \cite{huang2011adversarial, barreno2006can, barreno2010security} and is extended in \cite{munoz2017towards} to multiclass classification. 
% In the following sections, we outline the attacker's goal, knowledge, capability and strategy necessary to perform a powerful DoS poisoning attack.

% \subsubsection{Goal}\label{ss:goal}
% \cite{papernot2018sok} define adversarial goals in the context of machine learning attacks and provide examples for the attacker's motivation.
% Denial-of-Service poisoning attacks aim at violating a system's availability by preventing the user from access to a system's normal functionality. 
% The goal of these attacks is making the model inconsistent or unreliable in the target environment (for example to break a spam filter, as shown in \cite{nelson2008exploiting}).
% To achieve a general inconsistency over all samples and classes, an attacker will try to cause the misclassification of any sample (indiscriminate attack) as any of the classes different from the true label (error-generic attack).


% \subsubsection{Knowledge}\label{ss:knowledge}
% The attacker can have different levels of knowledge regarding the training data $D_{tr}$, feature set $X$, learning algorithm $M$ along with the objective function $L$ and parameters $w$ of the targeted system.
% Limited-knowledge attacks simulate a more realistic attack setting, where the training data or learning algorithm is unknown.
% In scenario, an attacker uses substitute datasets and models during poisoning. 
% Perfect-knowledge attacks, on the other hand, simulate an attacker that knows everything about the targeted system.
% As a defender, these attacks can be used to derive the worst-case performance degradation estimates.
% When evaluating our defence, we choose both a limited-knowledge attack (label flipping, c.f. Section~\ref{ss:flip_attack}) and a stronger perfect-knowledge attack (back-gradient optimization, c.f. Section~\ref{ss:bg_attack}).

% \subsubsection{Capability}\label{capability}
% The attacker's capability characterizes to what extent the machine learning mechanism and data can be manipulated.
% Usually, we assume that a dataset is crowd-sourced and that an attacker can introduce a certain percentage $p$ of adversarial data points into the training dataset.
% In order to create poison samples which are at least somewhat difficult to detect with outlier detection techniques and data pre-filtering, these poisoned samples should not take extreme values (both in feature and target space).
% Thus, the features of poison data usually do not exceed the minimum and maximum values of the corresponding features in benign data.

% \subsubsection{Strategy}\label{strategy}
% The attacker's goal is defined by an attacker objective function $A$, which maps a poisoned model with parameters $w^*$ and a validation dataset $D_{val}$ to a real number, i.e. $A(D_{val}, w^*) \in \mathbb{R}$.
% The data available to the attacker is divided into three disjoint sets:
% $D_p$ and $D_{tr}$ to poison and learn the model, $D_{val}$ to evaluate the impact of poison instances on test-time data.
% The attacker aims at finding poisoned instances $D^*_p$ such that $A$ is maximized on $D_{val}$ for a model trained on $D_{p}^* \cup D_{tr}$.
% Formally:
% \begin{equation}
% D_p^* \in \arg\max_{D_{p}} A(D_{val}, w^*) % = L(D_{val}, w^*)
% \label{eq:1}
% \end{equation}
% \begin{equation}
% s.t. \quad w^* \in \arg\min_{w \in W} L(D_{tr} \cup D_p, w)
% \label{eq:2}
% \end{equation}

% Problem~\ref{eq:1} is called 'outer problem', since it depends on the model parameters $w^*$, which are found during model training ('inner problem', Equation~\ref{eq:2}).
% Thus, finding a set of poison data $D^*_p$ which maximizes the attacker reward is a bi-level optimization problem.
% Note that for DoS poisoning attacks, maximizing the attacker's objective function $A$ is equivalent to maximizing the model loss $L$, thus $A = L$ in Equation~\ref{eq:1}.

% \subsection{DoS Poisoning via Label Flipping Attack}\label{ss:flip_attack}
% Compared to optimal attack strategies, the label flipping attack offers less flexibility, since the attacker only changes the label, but not the feature values of a given sample. 
% As a baseline attack, we consider Random Label Flipping, where the attacker selects a maximum percentage $p$ of instances at random from the training dataset and changes their labels to a class different from the original one \cite{paudice2018label}.
% This simple concept of label flipping describes a limited-knowledge attack, as it only requires the attacker to have access to the training dataset $D_{tr}$.

% \subsection{DoS Poisoning via Back-gradient Optimization Attack}\label{ss:bg_attack}
% In this section, we describe a perfect-knowledge back-gradient poisoning attack as presented in \cite{munoz2017towards}.
% The attack is characterized by iteratively adding poison samples into the training set.
% Every poison sample is initially assigned a class different from the original label. 
% The attack then repeats poisoning steps to modify the features of a malicious sample and increase its impact on the degradation of a model.
% Every poisoning step uses the concept of back-gradient optimization to derive $\nabla_{x_p}A$, which describes how the attacker's objective function varies with respect to a single poison instance $x_p$.
% The problem presented in Equations \ref{eq:1}, \ref{eq:2} can be solved through applying gradient ascent under the assumption that the loss function $L$ is differentiable with respect to $w$ and $x_p$. 
% %To understand how the attacker's objective function varies with respect to the poisoning point, we compute the gradient using the chain rule:\\
% %Thus, \cite{munoz2017towards} compute the required gradient using the chain rule.
% \begin{equation}
% \nabla_{x_p} A = \nabla_{x_p} L + \frac{\partial w}{\partial x_p} \nabla_w L
% \end{equation}
% Computing $\frac{\partial w}{\partial x_p}$ to obtain how the solution of the learning algorithm changes depending on the poison sample is challenging.
% \cite{munoz2017towards} discuss previous solutions of the bi-level optimization problem.
% Early poisoning attacks have replaced the inner problem with its stationary Karush-Kuhn-Tucker (KKT) conditions, but this approach can be prohibitively expensive in time and memory, especially for larger neural networks.
% Also, deriving proper stationary conditions involving all parameters is challenging.

% The approach presented in~\cite{munoz2017towards} replaces the inner optimization with a sequence of learning steps to smoothly update the parameters $w$. 
% After an incomplete optimization of the inner problem within $T$ iterations, the parameters $w_T$ can be used to compute the desired gradients of the outer problem.
% To avoid storing the whole training trajectory $w_1, ..., w_T$ along with the forward derivatives for back-propagation, \cite{munoz2017towards} propose to compute these parameters during the backward pass based on $w_T$ by reversing the steps of the learning algorithm.
% How to derive $\nabla_{x_p} A$ by reversing a gradient-descent procedure with a fixed number of epochs $T$ and a fixed step size is summarized in the pseudo-code algorithms presented in \cite{munoz2017towards}.

% While the current state-of-the-art approach based on KKT conditions requires solving one linear system per parameter and computationally demanding matrix multi layer perceptron generalizationoperations that scale in time as $O(|w|^3)$ and in memory as $O(|w|^2)$, the time complexity of back-gradient descent is in $O(T)$. This significantly reduces the complexity of computing the outer gradient and enables to evaluate the effectiveness of poisoning attacks against large neural networks and deep learning algorithms.

% To prove the effectiveness of this approach, an indiscriminate error-generic perfect-knowledge poisoning attack with back-gradient optimization is evaluated in \cite{munoz2017towards} on the datasets Spambase (spam email classification) and Ransomware (malware detection) against three machine learning algorithms: Multi-Layer-Perceptron (one hidden layer of 10 neurons), Logistic Regression and Adaline. By controlling only $15 \%$ of the training data, the classification error increased to around $30 \%$. They also show the applicability of the back-gradient attack algorithm to poison a deep neural network. When attacking the classification of MNIST using a convolutional neural network with $450000$ parameters by poisoning $1 \%$ of training instances, the classification error only slightly increases compared to random label flipping. They conclude that deep neural networks are more resilient against poisoning attacks, but leave this to a further investigation.

% \section{Poisoning Defence}\label{s:poisoning_defence}
% To introduce our approach, we outline the requirements of a feasible defence against DoS poisoning attacks. The system pipeline details how poisoned instances can be identified and removed from a given classification dataset. We conclude the following section on our defence by describing its improvements to related work.

% \subsection{Requirements}\label{ss:requirements}
% %We propose an easy-to-use defence against DoS data poisoning.
% Our easy-to-use and computationally efficient algorithm enables a fast identification and rejection of poison instances without any user inspection.
% At best, the defence should identify all poison instances in a dataset without previously knowing the exact fraction $p$ and without putting any further constraints on the dataset values.
% Our mechanism is not restricted to linear or binary classifiers and works especially well with neural networks.
% To detect and discard malicious instances crafted by the poisoning algorithm with back-gradient optimization, our defence only needs the model and data instances with labels. 
% This is the most general input necessary for every machine learning classification task and shows the applicability of our defence in any real world setting.
% The only constraint is that the number of poison instances should be smaller than the overall number of training instances, otherwise a distinction between benign and malicious data would not be possible. 
% We assume a maximum poison rate of $10\%$, which is already a high assumption for publicly available datasets.

% \subsection{System Pipeline}\label{system_pipeline}
% Our defence identifies poison instances and removes them from the dataset, while legitimate data remains in the dataset. 
% This approach is based on \cite{muller2019identifying}, who detect mislabeled instances in classification datasets.

% We define the following notation:
% Let $D$ be a dataset $D=(x,y)$, consisting of $N$ instances out of $C$ classes. 
% Input $x$ represents $N$ data instances of dimension $D$ while target $y$ represents $N$ data labels as one hot-encoded vectors of length $C$.
% Both $x$ and $y$ can be conveniently expressed in matrix notation.
% Finally, let $D^*_p \subseteq D$ be the set of poison instances, which is unknown to the defender.

% To identify these poison samples, we train a classifier $M$ on the given dataset $D=(x,y)$ and use the same classifier to obtain new class probabilities for $x$. 
% We then discard instances for which the class probability is small, which means that the classifier considers the original label extremely unlikely based on the feature distribution learned during training. 
% This works because there is still a significant majority of unpoisoned data in the training dataset.
% It is a reasonable assumption to make for crowd-sourced datasets, where a malicious individual can only introduce a small portion of malicious data.
% Nevertheless, we show in our experiments that our system works with up to $10$ percent of poison data in the training dataset.

% Formally, we design an indicator function $f \to \{0, 1\}$ where $f(d) = 1$ indicates that $d \in D$ is poisoned.
% We aim at maximizing the intersection between the true poisoned samples $D^*_p$ and $\{d \in D | f(d) = 1 \}$ while minimizing the intersection of $D^*_p$ and $\{d \in D | f(d) = 0 \}$.
% Our proposed algorithm is as follows.
% \begin{enumerate}
%     \itemsep0em
%     \item Given a dataset $D=(x,y)$ with possibly crafted poison instances, i.e. $D = D_{tr} \cup D^*_p$. We allow $D^*_p$ to be empty, as is the case when no attack is present.
%     \item Train model $M$ on the dataset $D$.
%     \item Reclassify training input $x$ using the trained model $M$ and obtain new class probabilities $M(x)=y'$.
%     \item Calculate for all $n\in \{0, ..., N-1\}$ the label likelihood $l_n$ that instance $x_n$ is assigned the original label $y_n$.
%     \begin{equation}
%     l_n := \langle y_n,y'_n \rangle = y'_{n_c}
%     \end{equation}
%     where $c$ is the non-zero valued index in the one-hot vector $y_n$.
%     \item Sort all training instances according to $l_n$ in ascending order. This yields a graph as presented in Figure~\ref{fig:back_gradient_poisoning_kneeplot}, where instances with small likelihood w.r.t their original label are on the left end of the plot.
%     \item Determine a threshold $k \in \{0, ..., N-1\}$ to distinguish between wrongly labeled poison data and correctly labeled benign data. 
%     We find this threshold by approximating the first derivative of $l_n$ over a sliding window, and simply choosing $k$ as the argmax. We motivate this in Section~\ref{ss:defence}.
%     \item Remove instances $D_p'$ where $l_i \leq l_k$ (i.e. left of the cutoff point) from the training set.
%     Retrain the model on $D - D_p'$.
%     \item Iteratively apply steps 3 to 7 until convergence.
% \end{enumerate}
% The intuition behind this algorithm is as follows:
% By computing the likelihood $l_n$, we estimate the probability that the given label is the true label.
% This requires a model $M$ which can generalize well even in the presence of adversarial data, such that it learns from the benign data instances what the poisoned instances' labels should be.
% We then sort the instances by $l_n$ and remove a portion which has very small $l_n$ (and thus likely has a wrong label, which indicates adversarial data).
% We retrain our model on the remaining data and iteratively re-evaluate the whole dataset.
% In our empirical evaluation in Section~\ref{s:empircal_eval}, we find that this approach reliably identifies poisoned instances with low false positive and false negative rates.

% On the choice of model $M$:
% It must be able to generalize well and not overfit the dataset, so that deviations from the overall distribution of a class can be easily found.
% Neural networks satisfy these requirements. 
% %Hence, we choose a dense feed forward neural network consisting of 3 layers and the binary or respectively categorical cross entropy loss.
% To prevent overfitting, we use an aggressive learning rate of 0.1 and impose early stopping on the loss with patience=10 and min\_delta=0.05.

% \subsection{Improvements to Related Work}
% With our system pipeline, we overcome fundamental restrictions of previous defences against data poisoning. While most attacks and defences focused on binary classification tasks and linear machine learning models, we provide a defence against multiclass poisoning attacks on neural networks.
% \cite{nelson2008exploiting} measure the impact of each training sample on the classifier's performance to determine and discard samples that decrease the accuracy. While this approach requires a step of retraining for every single sample, our defence only requires one full training of the model.
% Compared to clustering and outlier detection \cite{paudice2018detection, paudice2018label} our defence does not suffer from the curse of dimensionality \cite{Keogh2017} and is thus applicable in a learning environment with high dimensional data.
% Knowing the fraction of poison samples in the dataset is crucial for a good performance of robust logistic regression and classification in \cite{feng2014robust}. The biggest achievement of our defence is the identification and removal of poison samples from a training dataset without any knowledge of the fraction of poison samples and without any other user interaction.

% \section{Evaluation}\label{s:empircal_eval}
% The experimental evaluation presented in the following section shows the threat of data poisoning and the effectiveness of our defence. We run poisoning attacks with label flipping and back-gradient optimization on six numerical datasets and apply our defence to identify these crafted malicious samples.

% \subsection{Datasets}\label{ss:datasets}
% To demonstrate the behavior of back-gradient poisoning and the reliability of our poisoning defence, we choose six numerical datasets: One synthetic dataset of 2-dimensional \emph{points}, and six popular datasets to show the applicability in a real world environment.
% More specifically, we use \emph{iris}, \emph{wine} and \emph{breast cancer} from the \emph{sklearn} library \cite{scikit-learn} and \emph{spambase} and \emph{car} from the UCI Machine Learning Repository \cite{Dua:2019}.

% Table \ref{table:datasets} shows these datasets along with their original number of instances, features and classes. The algorithms were evaluated on datasets consisting of $|D_{tr}|$ benign train instances, $|D_p^*|$ poison instances, $|D_{val}|$ validation instances and $|D_{test}|$ test instances. For smaller datasets, we assumed that splitting the data available to the attacker would not improve the impact of poisoning, thus we decided to apply $D_{val}=D_{tr}$. Poisoning attacks on smaller training and validation datasets can suffer from a less powerful generalization of the error impact on the testing dataset, but still create valid poison samples for the evaluation of our defence.

% \begin{table}[h!]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% Name & Size & Classes & {$|D_{tr}|$} & \textbf{$|D_p^*|$} &  \textbf{$|D_{val}|$} & \textbf{$|D_{test}|$}\\
% \hline
% breast cancer & (569, 30) & 2 & 150 & 18 & 200 & 201\\
% car & (1728, 21) & 4 & 200 & 24 & 400 & 1103\\
% iris & (150, 4) & 3 & 100 & 12 & 100 & 38\\
% points & (560, 2) & 3 & 100 & 12 & 200 & 248\\
% spambase & (4601, 57) & 2 & 300 & 36 & 500 & 3765\\
% wine & (178, 13) & 3 & 100 & 12 & 100 & 66\\
% \hline
% \end{tabular}
% \caption{Datasets used in our empircal evaluation}
% \label{table:datasets}
% \end{table}

% \subsection{Attack}\label{ss:attack}
% We first provide a detailed investigation of poisoning neural networks (one hidden layer of 10 neurons) with label flipping and back-gradient optimization.

% Following the algorithm explained in Section \ref{s:poisoning_attack}, we craft poison samples and inject malicious instances $D_p^*$ into the training dataset in order to corrupt up to 10\% of all training samples.
% Poisoning with back-gradient optimization is constrained by ensuring that the values of a feature cannot exceed the minimum and maximum values of this feature in the clean dataset. 
% To obtain stable back-gradients we use 100 iterations for model training (incomplete optimization of the inner problem) and thus also 100 iterations for back-gradient optimization (outer problem).
% The loop for crafting a single poison sample terminates when there was no increase of the validation loss within the last three poisoning iterations.
% The label flipping attack is performed by simply assigning every poison sample a class different from the original label.

% To quantify the impact of these poisoning attacks, we report the model loss, model accuracy and the rotation of the decision surface (cosine distance) for varying degrees of data poisoning.
% For each dataset we craft poison samples that correspond to $12\%$ of the benign training instances, both via label flipping and back-gradient optimization attack.
% We then repeat our experiments with random subsets of these poison samples, and report averaged results.

% \begin{figure}[h!]
% \centering
% \begin{subfigure}[b]{0.495\textwidth}
% \includegraphics[width=\textwidth]{img/img_code/points/dataset=points_samples=100_poison_rate=0.1_xc_original=[-0.74_-1.18]_xc_result=[2.96_-3.7]_validation_loss_heatmap_step=0.png}
% \caption{The Loss}
% \label{fig:points_heat_map_loss}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.495\textwidth}
% \includegraphics[width=\textwidth]{img/img_code/points/dataset=points_samples=100_poison_rate=0.1_xc_original=[-0.74_-1.18]_xc_result=[2.96_-3.7]_validation_accuracy_heatmap_step=0.png}
% \caption{Accuracy}
% \label{fig:points_heat_map_accuracy}
% \end{subfigure}
% \caption{The trajectory of a malicious sample during a poisoning attack with back-gradient optimization. After initially switching the label from $2$ to $1$, the instance is moved from $x_p=[-0.74, -1.18]$ (region of smaller model loss) to $x_p=[2.96, -3.7]$ (region of higher model loss) by iteratively applying back-gradients.}
% \end{figure}

% We give a visual example of the back-gradient optimization attack in Figure \ref{fig:points_heat_map_loss} and \ref{fig:points_heat_map_accuracy}.
% These figures depict a dataset with three classes (shown as blue, red and green dots) over a two dimensional feature space.
% The black crosses represent a single poisoned data point over the course of 26 attack iterations.
% This poison sample is created by taking a legitimate data instance, flipping its label to a poison label (as indicated in the caption), and then iteratively moving it to a region where it will induce higher validation loss and lower validation accuracy.
% The effects of training a model on the normal data $D_{tr}$ plus a single poisoned instance $x_p$ are shown by the background color map, whose $x_1$, $x_2$ coordinates represent the coordinates of the poisoned instance $x_p$.
% To create the background plot, we partition the $x_1$, $x_2$ feature space into a grid, train a model for each poison instance on the grid, and plot validation loss and accuracy.
% This gives us the 'ground truth' with respect to how the poison sample should be changed in order to be maximally effective.
% We then execute the back-gradient attack and observe from Figure~\ref{fig:points_heat_map_loss} that it moves the adversarial data instance $x_p$ from regions of small validation loss (white) to regions of high validation loss (dark red).
% Figure~\ref{fig:points_heat_map_accuracy} presents the same setting, but the background contour now shows the validation accuracy of the model trained on the benign dataset plus the single poisoned point.
% We see that the back-gradient attack moves the data point from a region of high accuracy (dark red, center) to a region of lower accuracy (light red, bottom right).

% We can also evaluate the effectiveness of the attack by plotting the model's decision surface.
% Figure~\ref{fig:dec_borders_all} shows a \emph{points} classification task with no adversarial data poisoning, as well as data poisoning induced by the label flipping and back-gradient optimization attack.
% Observe how the attacks alter the decision surface and how model loss and accuracy are possibly deteriorated.

% Figures \ref{fig:car_loss}, \ref{fig:car_accuracy} and \ref{fig:car_cosine_distance} visualize the exemplary change of test loss, test accuracy and cosine distance when poisoning up to 10\% of the \emph{car} dataset. The impact of poisoning with back-gradient optimization on the test loss and test accuracy of all six datasets is displayed in Figure \ref{fig:all_datasets_loss} and Figure \ref{fig:all_datasets_accuracy}.
% Table \ref{table:back_gradient_attack_results} summarizes the averaged results of label flipping and back-gradient attacks and compares them to the test loss and test accuracy obtained from training on a clean dataset.
% The degradation of the performance of neural networks shows that especially poisoning attacks with back-gradient optimization pose a severe threat to machine learning algorithms and require an effective and efficient defence.

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[b]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{img/img_code/points/dataset=points_samples=112_poison_rate=0.1_decision_borders_Before poisoning attack_loss=0.299_accuracy=0.857.png}
%     \caption{Before poisoning attack}
%     \label{fig:decision_borders_before_poisoning}
%   \end{subfigure}
%   \hfill
%     \begin{subfigure}[b]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{img/img_code/points/dataset=points_samples=112_poison_rate=0.1_decision_borders_After label flipping_loss=0.561_accuracy=0.777.png}
%     \caption{After label flipping}
%     \label{fig:decision_borders_after_flipping}
%   \end{subfigure}
%     \begin{subfigure}[b]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{img/img_code/points/dataset=points_samples=112_poison_rate=0.1_decision_borders_After back-gradient optimization_loss=0.550_accuracy=0.795.png}
%     \caption{After back-gradient optimization}
%     \label{fig:decision_borders_after_poisoning}
%   \end{subfigure}
%   \caption{The effect of introducing 12 poison instances into a classification dataset. 
%   The left figure shows the unpoisoned dataset, where the bold crosses indicate the data instances to be changed during the upcoming attack.
%   The middle figure shows the impact on the decision surface when the flip attack is applied. Note that there is only small change of the decision surface.
%   The right figure shows the decision surface after the back-gradient attack.
%   Note that not only the labels, but also the feature values of the poison data have changed. The decision surface is considerably altered.}
%   %, and model loss and accuracy have been significantly deteriorated.
%   \label{fig:dec_borders_all}
% \end{figure}


% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[b]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{img/img_code/car/dataset=car_n=200_k=24_poison_rate=0.1_folds=10_mean_loss_plot.png}
%     \caption{Test loss}
%     \label{fig:car_loss}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{img/img_code/car/dataset=car_n=200_k=24_poison_rate=0.1_folds=10_mean_accuracy_plot.png}
%     \caption{Test accuracy}
%     \label{fig:car_accuracy}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{img/img_code/car/dataset=car_train_samples=200_poison_rate=0.1_train_cosine_distance_plot.png}
%     \caption{Cosine distance}
%     \label{fig:car_cosine_distance}
%   \end{subfigure}
%   \caption{Degradation of a model's performance when iteratively adding crafted poison samples into the \emph{car} training dataset. The figure on the left shows the increase of test loss (attacker reward) while the figure in the middle shows the decrease of test accuracy when training a model on increasingly poisoned data. To visualize the impact of poisoning on the model itself, the right figure depicts the cosine distance of model parameters $w$ obtained from training on a clean and poisoned dataset.}
% \end{figure}

% \begin{table}
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
% \hline
% dataset & \multicolumn{3}{c|}{cosine distance} & \multicolumn{3}{c|}{test loss} & \multicolumn{3}{c|}{test accuracy}\\
% & clean & flipped & back-grad & clean & flipped & back-grad & clean & flipped & back-grad\\
% \hline
% breast cancer &                    0.0 &                     0.16 &                0.20 &             0.11 &               0.29 &          0.35 &                 0.97 &                   0.89 &              0.86 \\
% car &                    0.0 &                     0.12 &                0.18 &             0.30 &               0.55 &          0.75 &                 0.87 &                   0.80 &              0.73 \\
% iris &                    0.0 &                     0.05 &                0.12 &             0.08 &               0.23 &          0.29 &                 1.00 &                   0.92 &              0.97 \\
% points &                    0.0 &                     0.06 &                0.14 &             0.23 &               0.31 &          0.34 &                 0.95 &                   0.94 &              0.89 \\
% spambase &                    0.0 &                     0.16 &                0.17 &             0.43 &               0.50 &          0.65 &                 0.91 &                   0.86 &              0.82 \\
% wine &                    0.0 &                     0.12 &                0.19 &             0.07 &               0.31 &          0.31 &                 0.98 &                   0.91 &              0.88 \\
% \hline\hline
% \textbf{mean} &                    \textbf{0.0} &                     \textbf{0.11} &                \textbf{0.17} &             \textbf{0.20} &               \textbf{0.36} &          \textbf{0.45} &                 \textbf{0.95} &                   \textbf{0.89} &              \textbf{0.86} \\
% \hline
% \end{tabular}
% \caption{Results of applying the label flipping and back-gradient attack on datasets, averaged over 15 runs. Poisoning 10\% of the training data causes a significant change of the model parameters (cosine distance) and degrades the model's performance with respect to the test loss and test accuracy.}
% \label{table:back_gradient_attack_results}
% \end{table}

% \subsection{Defence}\label{ss:defence}
% We now apply the defence presented in Section \ref{s:poisoning_attack} to the six poisoned datasets.
% For every dataset we obtain a so-called knee plot after sorting all training instances according to their likelihood $l_n$ of being assigned the original label.
% Figure~\ref{fig:back_gradient_poisoning_kneeplot} gives an example for the \emph{breast cancer} dataset.
% While the red line shows the true rate of poison samples in our training dataset (p=10\%), the green line is the model's estimate of the poisoning rate.
% This estimate $\hat{p}$ is selected as the highest increase in $l_n$ over $n$.
% We compute $\hat{p}$ using a sliding window over $l_n$ in order to approximate the first derivative of $l_n$, and choose the argmax. After applying our system pipeline twice, we receive the right plot of label likeliness.

% The intuition behind this approach is as follows:
% The poison estimate $\hat{p}$ separates values of low and high label likelihood $l_n$. 
% Low values indicate a mismatch between feature and target value, which may indicate poisoned data.
% An oracle would assign benign data a label likelihood of $l_n = 1$ and poisoned data a likelihood of $l_n = 0$.
% Thus, the obvious choice of threshold would be the point of discontinuity in $l_n$.
% Since we need to work with an imperfect classifier instead of an oracle, the discontinuity is not as pronounced.
% However, the largest derivative is a solid approximation which we find to work well.

% To assess the reliability and effectiveness of identifying and removing poison samples from a training dataset, we compute false positives and false negatives.
% False positives (FP) correspond to the non-poison samples among the samples ordered left of the threshold that our classifier wrongly assumes to be poisoned and will be discarded from the training dataset.
% False negatives (FN) correspond to the poison samples among the samples ordered right of the threshold that our classifier wrongly assumes to be benign and will remain in the training dataset.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\textwidth]{img/img_code/breast_cancer/dataset=breast_cancer__poison_rate=0.1_knee_plot_labelfix_iterations=2_fold=8.png}
%     \caption{A 'knee-plot' of label likelihood values $l_n$ (blue), sorted in ascending order.
%     The x-axis lists the sorted 166 instances of the \emph{breast cancer} training dataset, while the y-axis shows the corresponding label likelihood-values $l_n$.
%     The red line represents the true fraction of poison samples (10\%), while the green line represents the fraction estimated by our defence algorithm.
%     Our defence is not only accurate in estimating this percentage, but also identifies individual instances with a low $FPR=0.02$ and a low $FNR=0.01$.
%     The poisoned test loss is reduced from $0.33$ to $0.13$, and the test accuracy is increased from $0.89$ to $0.95$.}
%     \label{fig:back_gradient_poisoning_kneeplot}
% \end{figure}

% \subsubsection{Results}
% We apply our defence to two scenarios: Data poisoned with the \emph{Label Flipping} attack, and the \emph{Back-gradient Optimization} attack.
% Table \ref{tab:back_gradient_defence_overview} presents the averaged results of our defence after applying the system pipeline twice.
% We identify poisoned instances with an averaged FPR=0.02 and FNR=0.02, significantly outperforming a random baseline where both FPR, FNR = 0.09.
% Note that our defence does not have knowledge of the poison rate.
% A more detailed investigation is provided in the appendix, where Table~\ref{tab:back_gradient_defence_results} and Table \ref{tab:label_flipping_defence_results} show the results for datasets and poisoning rates individually.

% For additional evaluation, we use Receiver Operating Characteristics (ROC) curves known from the field of information retrieval \cite{zuva2012evaluation}.
% Figure~\ref{fig:roc_curves} presents the ROC for our six datasets and compares them to a random baseline, which is consistently outperformed.

% \begin{table}[h!]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
% \hline
% dataset &$\hat{p}$& \multicolumn{2}{c|}{FP} & \multicolumn{2}{c|}{FN} & \multicolumn{2}{c|}{test loss} & \multicolumn{2}{c|}{test accuracy}\\
%  & & random & defence & random & defence & before & after & before & after\\
% \hline
% breast cancer &   0.103 &                       0.089 &                0.023 &                       0.089 &                0.010 &              0.33 &             0.13 &                  0.89 &                 0.95 \\
% car           &   0.138 &                       0.089 &                0.061 &                       0.089 &                0.018 &              0.75 &             0.79 &                  0.73 &                 0.80 \\
% iris          &   0.093 &                       0.086 &                0.002 &                       0.095 &                0.008 &              0.28 &             0.08 &                  0.96 &                 1.00 \\
% points        &   0.100 &                       0.086 &                0.033 &                       0.095 &                0.032 &              0.35 &             0.27 &                  0.89 &                 0.93 \\
% spambase      &   0.043 &                       0.087 &                0.018 &                       0.081 &                0.064 &              0.65 &             0.71 &                  0.82 &                 0.84 \\
% wine          &   0.100 &                       0.088 &                0.002 &                       0.097 &                0.001 &              0.35 &             0.08 &                  0.86 &                 0.97 \\
% \hline\hline
% \textbf{mean}          &   \textbf{0.096} &                       \textbf{0.088} &                \textbf{0.023} &                       \textbf{0.091} &                \textbf{0.022} &              \textbf{0.45} &             \textbf{0.34} &                  \textbf{0.86} &                 \textbf{0.92} \\
% \hline
% \end{tabular}
% \caption{Results of our proposed defence applied on datasets poisoned with the back-gradient attack, averaged over 15 runs. The datasets contain 10\% poison samples each.
% The column $\hat{p}$ shows the poison rate estimated by the defence algorithm (the true poison rate $p=0.1$ is unknown to the defender).
% The next two columns compare FPR and FNR of the defence algorithm against a random baseline, which is consistently outperformed.
% Additionally, test loss and accuracy improve considerably when using the defence on the poisoned dataset, as shown in the last two columns.
% }
% \label{tab:back_gradient_defence_overview}
% \end{table}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/img_code/all_datasets_poison_rate=0.1_roc_plot.png}
%     \caption{ROC curves averaged over 15 runs, obtained by applying our defence on six datasets poisoned with the \emph{back-gradient} attack.
%     The x-axis presents the fraction of false positive samples (benign data) while the y-axis presents the fraction of true positive samples (poison data) at varying  thresholds. 
%     The random baseline (grey line) is consistently outperformed.}
%     \label{fig:roc_curves}
% \end{figure}

% \section{Conclusion and Future Work}
% In this paper, we present a new principled defence against DoS poisoning attacks.
% Our proposed mechanism can identify and discard malicious instances from a classification dataset, either by selecting a threshold automatically, or by sorting the instances for efficient triage by a human expert.
% While previous work has mostly used clustering and outlier detection against poisoning attacks, we re-evaluate the training samples by the poisoned classifier.
% The experimental evaluation on six numerical datasets has shown that our approach consistently outperforms the random baseline.

% We identify the following possibility for future work:
% First, our defence could be evaluated on a wider class of machine learning algorithms.
% However, as long as the algorithm generalizes sufficiently, our approach should be transferable.
% Second, our experimental analysis could be extended to image and time-series data.
% Finally, we would like establish the reclassification of samples as a basic defence approach and explore new ways of threshold selection.

% \appendix
% \section{Appendix}
% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}
%     \includegraphics[width=\textwidth]{img/img_code/all_datasets_poison_rate=0.1_back_gradient_loss_plot.png}
%     \caption{Loss}
%     \label{fig:all_datasets_loss}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.49\textwidth}
%     \includegraphics[width=\textwidth]{img/img_code/all_datasets_poison_rate=0.1_back_gradient_accuracy_plot.png}
%     \caption{Accuracy}
%     \label{fig:all_datasets_accuracy}
%   \end{subfigure}
%   \caption{Back-gradient attack against six datasets. The results show how the performance of a model is degraded when poisoning up to 10\% of the training data.
%   While the x-axis lists the poisoning rate, the y-axis represents the percentage change of test loss in the left plot and the percentage change of test accuracy in the right plot. There is a clear correlation between increasing the attacker's objective function (loss) and decreasing the model's prediction accuracy.}
% \end{figure}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
% \hline
% dataset & $p$ & $\hat{p}$ & \multicolumn{2}{c|}{FP} & \multicolumn{2}{c|}{FN} & \multicolumn{2}{c|}{test loss} & \multicolumn{2}{c|}{test accuracy}\\
%  & & & defence & random & defence & random & before & after & before & after\\
% \hline
% breast cancer & 0.00 &   0.007 &                       0.000 &                0.007 &                       0.007 &                0.000 &              0.11 &             0.09 &                  0.97 &                 0.97 \\
%      & 0.03 &   0.036 &                       0.030 &                0.010 &                       0.037 &                0.006 &              0.20 &             0.11 &                  0.94 &                 0.96 \\
%      & 0.05 &   0.052 &                       0.047 &                0.013 &                       0.053 &                0.012 &              0.24 &             0.12 &                  0.92 &                 0.95 \\
%      & 0.10 &   0.101 &                       0.086 &                0.023 &                       0.086 &                0.012 &              0.35 &             0.14 &                  0.86 &                 0.95 \\
% \hline
% car & 0.00 &   0.040 &                       0.000 &                0.040 &                       0.005 &                0.000 &              0.30 &             0.52 &                  0.87 &                 0.85 \\
%      & 0.03 &   0.072 &                       0.028 &                0.046 &                       0.033 &                0.003 &              0.51 &             0.57 &                  0.79 &                 0.83 \\
%      & 0.05 &   0.103 &                       0.048 &                0.060 &                       0.048 &                0.004 &              0.60 &             0.66 &                  0.77 &                 0.82 \\
%      & 0.10 &   0.140 &                       0.088 &                0.066 &                       0.088 &                0.020 &              0.74 &             0.81 &                  0.73 &                 0.79 \\
% \hline
% iris & 0.00 &   0.030 &                       0.000 &                0.030 &                       0.010 &                0.000 &              0.08 &             0.12 &                  1.00 &                 0.92 \\
%      & 0.03 &   0.026 &                       0.026 &                0.001 &                       0.036 &                0.003 &              0.16 &             0.09 &                  0.97 &                 1.00 \\
%      & 0.05 &   0.043 &                       0.044 &                0.000 &                       0.053 &                0.005 &              0.20 &             0.08 &                  0.97 &                 1.00 \\
%      & 0.10 &   0.093 &                       0.092 &                0.002 &                       0.101 &                0.008 &              0.27 &             0.08 &                  0.96 &                 1.00 \\
% \hline
% points & 0.00 &   0.050 &                       0.000 &                0.050 &                       0.010 &                0.000 &              0.23 &             0.28 &                  0.95 &                 0.94 \\
%      & 0.03 &   0.066 &                       0.028 &                0.042 &                       0.038 &                0.005 &              0.28 &             0.27 &                  0.95 &                 0.94 \\
%      & 0.05 &   0.071 &                       0.043 &                0.037 &                       0.052 &                0.014 &              0.28 &             0.26 &                  0.94 &                 0.94 \\
%      & 0.10 &   0.100 &                       0.091 &                0.032 &                       0.100 &                0.031 &              0.35 &             0.27 &                  0.89 &                 0.93 \\
% \hline
% spambase & 0.00 &   0.017 &                       0.000 &                0.017 &                       0.003 &                0.000 &              0.43 &             0.52 &                  0.91 &                 0.91 \\
%      & 0.03 &   0.028 &                       0.031 &                0.017 &                       0.031 &                0.018 &              0.50 &             0.55 &                  0.88 &                 0.89 \\
%      & 0.05 &   0.038 &                       0.047 &                0.020 &                       0.047 &                0.030 &              0.53 &             0.61 &                  0.86 &                 0.88 \\
%      & 0.10 &   0.048 &                       0.090 &                0.018 &                       0.084 &                0.060 &              0.64 &             0.72 &                  0.82 &                 0.84 \\
% \hline
% wine & 0.00 &   0.010 &                       0.000 &                0.010 &                       0.010 &                0.000 &              0.07 &             0.06 &                  0.98 &                 0.97 \\
%      & 0.03 &   0.024 &                       0.028 &                0.000 &                       0.038 &                0.005 &              0.18 &             0.08 &                  0.93 &                 0.97 \\
%      & 0.05 &   0.043 &                       0.047 &                0.001 &                       0.056 &                0.006 &              0.23 &             0.09 &                  0.91 &                 0.97 \\
%      & 0.10 &   0.102 &                       0.087 &                0.004 &                       0.096 &                0.001 &              0.35 &             0.07 &                  0.86 &                 0.98 \\
% \hline
% \end{tabular}
% \caption{Results of applying our proposed defence on datasets poisoned with the back-gradient attack, averaged over 15 runs. The datasets contain up to 10\% poison samples each.
% The column $p$ shows the real poison rate, while $\hat{p}$ shows the poison rate estimated by the defence algorithm.}
% \label{tab:back_gradient_defence_results}
% \end{table}


% \begin{table}[h!]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
% \hline
% dataset & $p$ & $\hat{p}$ & \multicolumn{2}{c|}{FP} & \multicolumn{2}{c|}{FN} & \multicolumn{2}{c|}{test loss} & \multicolumn{2}{c|}{test accuracy}\\
%  & & & defence & random & defence & random & before & after & before & after\\
% \hline
% breast cancer & 0.00 &   0.007 &                       0.000 &                0.007 &                       0.007 &                0.000 &              0.11 &             0.09 &                  0.97 &                 0.97 \\
%      & 0.03 &   0.042 &                       0.031 &                0.013 &                       0.038 &                0.003 &              0.19 &             0.10 &                  0.93 &                 0.96 \\
%      & 0.05 &   0.062 &                       0.048 &                0.015 &                       0.054 &                0.004 &              0.22 &             0.10 &                  0.92 &                 0.96 \\
%      & 0.10 &   0.104 &                       0.088 &                0.021 &                       0.088 &                0.007 &              0.33 &             0.12 &                  0.86 &                 0.95 \\
% \hline
% car & 0.00 &   0.040 &                       0.000 &                0.040 &                       0.005 &                0.000 &              0.30 &             0.52 &                  0.87 &                 0.85 \\
%      & 0.03 &   0.067 &                       0.027 &                0.044 &                       0.032 &                0.006 &              0.41 &             0.57 &                  0.83 &                 0.84 \\
%      & 0.05 &   0.087 &                       0.049 &                0.052 &                       0.049 &                0.013 &              0.46 &             0.63 &                  0.81 &                 0.82 \\
%      & 0.10 &   0.132 &                       0.090 &                0.058 &                       0.090 &                0.021 &              0.54 &             0.72 &                  0.80 &                 0.81 \\
% \hline
% iris & 0.00 &   0.030 &                       0.000 &                0.030 &                       0.010 &                0.000 &              0.08 &             0.12 &                  1.00 &                 0.92 \\
%      & 0.03 &   0.026 &                       0.028 &                0.001 &                       0.038 &                0.003 &              0.13 &             0.08 &                  0.98 &                 1.00 \\
%      & 0.05 &   0.042 &                       0.045 &                0.001 &                       0.054 &                0.006 &              0.17 &             0.10 &                  0.95 &                 0.99 \\
%      & 0.10 &   0.072 &                       0.090 &                0.000 &                       0.099 &                0.027 &              0.23 &             0.12 &                  0.90 &                 0.96 \\
% \hline
% points & 0.00 &   0.050 &                       0.000 &                0.050 &                       0.010 &                0.000 &              0.23 &             0.28 &                  0.95 &                 0.94 \\
%      & 0.03 &   0.071 &                       0.029 &                0.046 &                       0.039 &                0.004 &              0.24 &             0.27 &                  0.95 &                 0.94 \\
%      & 0.05 &   0.085 &                       0.043 &                0.044 &                       0.053 &                0.007 &              0.26 &             0.27 &                  0.95 &                 0.94 \\
%      & 0.10 &   0.130 &                       0.089 &                0.047 &                       0.098 &                0.017 &              0.31 &             0.28 &                  0.92 &                 0.93 \\
% \hline
% spambase & 0.00 &   0.017 &                       0.000 &                0.017 &                       0.003 &                0.000 &              0.43 &             0.52 &                  0.91 &                 0.91 \\
%      & 0.03 &   0.022 &                       0.030 &                0.012 &                       0.030 &                0.020 &              0.46 &             0.52 &                  0.89 &                 0.89 \\
%      & 0.05 &   0.033 &                       0.049 &                0.014 &                       0.049 &                0.029 &              0.48 &             0.55 &                  0.88 &                 0.89 \\
%      & 0.10 &   0.053 &                       0.089 &                0.019 &                       0.083 &                0.056 &              0.54 &             0.62 &                  0.85 &                 0.87 \\
% \hline
% wine & 0.00 &   0.010 &                       0.000 &                0.010 &                       0.010 &                0.000 &              0.07 &             0.06 &                  0.98 &                 0.97 \\
%      & 0.03 &   0.020 &                       0.028 &                0.000 &                       0.038 &                0.009 &              0.21 &             0.11 &                  0.93 &                 0.96 \\
%      & 0.05 &   0.033 &                       0.045 &                0.001 &                       0.055 &                0.016 &              0.20 &             0.13 &                  0.92 &                 0.96 \\
%      & 0.10 &   0.074 &                       0.086 &                0.000 &                       0.095 &                0.025 &              0.28 &             0.16 &                  0.91 &                 0.95 \\
% \hline
% \end{tabular}
% \caption{Results of applying our proposed defence on datasets poisoned with the label flipping attack, averaged over 15 runs. The datasets contain up to 10\% poison samples each.
% The column $p$ shows the real poison rate, while $\hat{p}$ shows the poison rate estimated by the defence algorithm.}
% \label{tab:label_flipping_defence_results}
% \end{table}

% \bibliographystyle{unsrt}
% \bibliography{references}

% \end{document}

